On length measures of planar closed curves and the comparison of convex shapes

In this paper, we revisit the notion of length measures associated to planar closed curves. These are a special case of area measures of hypersurfaces which were introduced early on in the field of convex geometry. The length measure of a curve is a measure on the circle $\mathbb{S}^1$ that intuitively represents the length of the portion of curve which tangent vector points in a certain direction. While a planar closed curve is not characterized by its length measure, the fundamental Minkowski-Fenchel-Jessen theorem states that length measures fully characterize convex curves modulo translations, making it a particularly useful tool in the study of geometric properties of convex objects. The present work, that was initially motivated by problems in shape analysis, introduces length measures for the general class of Lipschitz immersed and oriented planar closed curves, and derives some of the basic properties of the length measure map on this class of curves. We then focus specifically on the case of convex shapes and present several new results. First, we prove an isoperimetric characterization of the unique convex curve associated to some length measure given by the Minkowski-Fenchel-Jessen theorem, namely that it maximizes the signed area among all the curves sharing the same length measure. Second, we address the problem of constructing a distance with associated geodesic paths between convex planar curves. For that purpose, we introduce and study a new distance on the space of length measures that corresponds to a constrained variant of the Wasserstein metric of optimal transport, from which we can induce a distance between convex curves. We also propose a primal-dual algorithm to numerically compute those distances and geodesics, and show a few simple simulations to illustrate the approach.

==> header.tex <==
\usetheme{default}
\makeatletter


%%%% PACKAGE

%\usepackage{hyperref}

%Police et encodage
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
%\usepackage[T1]{fontenc}
%\usepackage{lmodern}
\usepackage{dsfont}
\usepackage{cancel}

%\usepackage{subcaption}
\usepackage{xcolor,colortbl}
\usepackage{graphicx,xmpmulti}
%\usepackage{diagbox,calc,soul}
\usepackage{calc,soul}
%\usepackage{tikz}
%\usetikzlibrary{calc,fadings,decorations.pathmorphing,decorations.pathreplacing,matrix,arrows,decorations.text,positioning,decorations.markings}
\usepackage{pgfplots}
%\usepgfplotslibrary{patchplots} 

\usepackage{ragged2e}
\justifying

\usepackage{amsmath}
\usepackage{amsbsy}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amscd}
\usepackage{amsthm}
\usepackage{epsfig}
\usepackage{algorithm,algorithmic}
\usepackage{appendix}
\usepackage{tikz-cd}
\usepackage{diagbox}
%\usepackage{mathtools}

\theoremstyle{definition}
\newtheorem{defi}{Definition}[section]
\newtheorem{remark}[defi]{Remark}
%\newtheorem{hyp}{Assumption}[section]

\theoremstyle{plain}
%\newtheorem{cor}[defi]{Corollary}
\newtheorem{thm}[defi]{Theorem}
\newtheorem{property}{Property}
\newtheorem{proposition}{Proposition}


%%%% ALIAS


\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\sabs}[1]{\lvert#1\rvert}
\providecommand{\babs}[1]{\bigg\lvert#1\bigg\rvert}
\providecommand{\Babs}[1]{\Big\lvert#1\Big\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}
\providecommand{\bnorm}[1]{\bigg\lVert#1\bigg\rVert}
\providecommand{\snorm}[1]{\lVert#1\rVert}
\providecommand{\Bnorm}[1]{\Big\lVert#1\Big\rVert}
\providecommand{\prs}[1]{\left\langle #1\right\rangle}
\providecommand{\sprs}[1]{\langle #1\rangle}
\providecommand{\bprs}[1]{\bigg\langle #1\bigg\rangle}
\providecommand{\Bprs}[1]{\Big\langle #1\Big\rangle}

\providecommand{\eg}{\textit{e.g} }
\providecommand{\cf}{\textit{c.f} }
\providecommand{\ie}{\textit{i.e} }
\providecommand{\bV}{\mathcal{V}}
\providecommand{\ppi}{\ensuremath{\boldsymbol{\pi}} }
\providecommand{\BV}{\ensuremath{\boldsymbol{\bV}} }
\providecommand{\R}{\mathbb{R}}
\providecommand{\Sp}{\mathbb S}
\DeclareMathOperator{\mdiv}{div}
\providecommand{\F}{\mathcal{F}}
\providecommand{\HH}{\mathcal{H}}
\providecommand{\MM}{\mathcal{M}}
\renewcommand{\P}{\mathbb{P}}
\providecommand{\PP}{\mathcal{P}}
\providecommand{\Z}{\mathbb{Z}}
\providecommand{\bZ}{\ensuremath{\boldsymbol{Z}}}%\providecommand{\bZ}{\mathbf{Z}}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\1}{\mathds{1}}
\newcommand{\one}{\ensuremath{\boldsymbol{1}} }
\providecommand{\Aa}{\ensuremath{\boldsymbol{a}} }
\renewcommand{\b}{\ensuremath{\boldsymbol{b}} }
\providecommand{\blambda}{\ensuremath{\boldsymbol{\lambda}} }
\providecommand{\y}{\ensuremath{\boldsymbol{y}} }
\providecommand{\p}{\ensuremath{\boldsymbol{p}} }
\providecommand{\N}{\mathbb{N}}
\providecommand{\C}{\mathbb{C}}
\providecommand{\CC}{\mathcal{C}}
\providecommand{\Sh}{\R^{k\times 2}}         
\providecommand{\X}{\mathbf{X}}
\providecommand{\Y}{\ensuremath{\boldsymbol{Y}} }%{\mathbf{Y}}%
\providecommand{\G}{\mathcal{G}}
\renewcommand{\S}{\mathbb{S}}
\providecommand{\bk}{\ensuremath{\boldsymbol{k}} }
\providecommand{\bh}{\boldsymbol{h}}
%\providecommand{\ba}{\mathbf{a}}
\providecommand{\m}{\mathrm{m}}
\providecommand{\bI}{\mathbf{I}}
\providecommand{\bsig}{\mathbf{\Sigma}}
\providecommand{\V}{\mathbf{V}}
\providecommand{\A}{\mathbf{A}}
\renewcommand{\AA}{\mathcal{A}}
\providecommand{\U}{\mathbf{U}}
\providecommand{\B}{\mathbf{B}}

\providecommand{\PPP}{\R^J\times[-\pi,\pi[^J\times\R^{2J}}
\providecommand{\T}{\mathbf{T}}
\providecommand{\TT}{\mathbb{T}}
\providecommand{\bY}{\mathbf{Y}}
\newcommand{\bSigma}{\ensuremath{\boldsymbol{\Sigma}} }
\newcommand{\bTheta}{\ensuremath{\boldsymbol{\Theta}} }
\newcommand{\btheta}{\ensuremath{\boldsymbol{\theta}} }
\newcommand{\btau}{\ensuremath{\boldsymbol{\tau}} }
\newcommand{\beps}{\ensuremath{\boldsymbol{\varepsilon}} }
\newcommand{\g}{\ensuremath{\boldsymbol{g}} }
\newcommand{\x}{\ensuremath{\boldsymbol{x}} }
\newcommand{\h}{\ensuremath{\boldsymbol{h}} }
\newcommand{\f}{\ensuremath{\boldsymbol{f}} }
\newcommand{\bJ}{\ensuremath{\boldsymbol{J}} }
\newcommand{\bvarepsilon}{\ensuremath{\boldsymbol{\varepsilon}} }
\providecommand{\balpha}{\ensuremath{\boldsymbol{\alpha}} }
\newcommand{\bzeta}{\ensuremath{\boldsymbol{\zeta}} }
\newcommand{\Tau}{\ensuremath{\boldsymbol{\mathcal T }}}
\providecommand{\quo}{\ensuremath{\X\slash\G} }

\def\Meas{\mathcal{M}_f(F)}
\def\MeasX{\mathcal{M}^X}
\def\MeasXC{\mathcal{M}^{X,C}}
\def\one{\mathbf{1}}
\def\eJ{\tilde{J}}
\def\X{{\mathcal X_0}}
\def\XX{{\mathcal X}}
\def\Haus{\mathcal{H}}
\def\sgn{\text{sgn}}
\def\Vol{\text{Vol}}
\def\df{\delta\!f}
\def\FB{\mathcal F}
\def\Cat{\text{Cat}}
\def\vol{\text{vol}}

\providecommand{\E}{\mathbb{E}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Card}{Card}
\DeclareMathOperator{\cov}{Cov}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\diag}{Diag}
\DeclareMathOperator*{\sign}{sgn}
\DeclareMathOperator{\tr}{tr}  
\DeclareMathOperator{\Jac}{Jac}
\providecommand{\LL}{\mathcal{L}}
\DeclareMathOperator*{\supp}{supp}

%%%% TOC

\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}
    
%%%% BEAMER    
    
\setbeamertemplate{navigation symbols}{}

\definecolor{mblack}{RGB}{0,0,0}
\definecolor{mwhite}{RGB}{255,255,255}
\setbeamercolor{ftcolor}{bg=mwhite,fg=mblack}
\defbeamertemplate*{footline}{}
{%
  \begin{beamercolorbox}[ht=2ex,dp=0.75ex,right]{ftcolor}
\insertframenumber/\inserttotalframenumber\hskip2ex \hspace*{.1ex}
  \end{beamercolorbox}%
}

%\setbeamertemplate{frametitle}
%{%
%\insertsubsectionnumber. \insertsubsectionhead~: {\mdseries \insertframetitle}
%}
\setbeamertemplate{blocks}[rounded][shadow=false]

\setbeamertemplate{section in toc}
{\inserttocsectionnumber. ~ \inserttocsection \\}

\setbeamertemplate{subsection in toc}
{\hspace{0.8cm} \inserttocsectionnumber.\inserttocsubsectionnumber. ~ \inserttocsubsection \\}

\setbeamertemplate{section in head/foot}
{\insertsectionheadnumber. \insertsectionhead}

\setbeamertemplate{subsection in head/foot}
{\insertsectionheadnumber.\insertsubsectionheadnumber. \insertsubsectionhead}

\setbeamertemplate{subsubsection in head/foot}
{\insertsectionheadnumber.\insertsubsectionheadnumber. \insertsubsubsectionheadnumber. \insertsubsubsectionhead}

%\setbeamertemplate{frametitle}{\insertframetitle}
\definecolor{greyone}{RGB}{77,77,77}
\definecolor{dgreen}{RGB}{0,100,0}
\setbeamercolor{hdcolor}{fg=white,bg=greyone}

\defbeamertemplate*{headline}{}
{%
  \begin{beamercolorbox}[wd=\paperwidth,ht=1.8em,dp=5ex,center]{hdcolor}%
	\vspace*{-.2cm}\strut{\bf\large \thesection~\insertsectionhead :} {\normalsize \insertsubsectionhead} \strut
	%\insertsubsectionnavigationhorizontal{.95\paperwidth}{}{}%\\
	  %\vspace*{-.2cm}\strut{\bf\large \thesection.\thesubsection. \insertsubsectionhead~: } {\normalsize \insertsubsubsectionhead} \strut
 \end{beamercolorbox}%
}
%\defbeamertemplate*{headline}{}
%{%
  %\begin{beamercolorbox}[ht=3ex,dp=0.75ex,center]{section in head/foot}%
	%\insertsectionnavigationhorizontal{.95\paperwidth}{}{}%\\
  %\end{beamercolorbox}%
%}
%Should use subcaptio...
%\usepackage{etoolbox}% http://ctan.org/pkg/etoolbox
%\AtBeginEnvironment{figure}{\setcounter{subfigure}{0}}% Resets subfigure counter at start of figure environment

\DeclareUnicodeCharacter{00A0}{~}

% Block

\setbeamertemplate{blocks}[shadow=false]

\setbeamercolor{block title}{fg=black,bg=gray!50}        % titre block normal 
\setbeamercolor{block body}{fg=black,bg=gray!10}      % corps block normal
\setbeamercolor{block body alerted}{fg=black,bg=red!10}   % idem pour un block alerte
\setbeamercolor{block title alerted}{fg=black,bg=red!50}   % idem pour un block alerte

%\usepackage[labelformat=empty]{caption}
%\setlength{\abovecaptionskip}{0pt}

%\makeatletter
%\renewcommand{\fnum@figure}{\footnotesize{Fig.}}
%\makeatother

\newenvironment{mylist}[2]{\begin{list}{#1}{\renewcommand{\makelabel}{\bfseries}}#2}{\end{list}
}

\newcommand\rst[2]{{#1}_{\restriction_{#2}}}

\makeatother

